Pointwise tube formulas for fractal sprays and self-similar tilings with arbitrary generators

In a previous paper by the first two authors, a tube formula for fractal sprays was obtained which also applies to a certain class of self-similar fractals. The proof of this formula uses distributional techniques and requires fairly strong conditions on the geometry of the tiling (specifically, the inner tube formula for each generator of the fractal spray is required to be polynomial). Now we extend and strengthen the tube formula by removing the conditions on the geometry of the generators, and also by giving a proof which holds pointwise, rather than distributionally. Hence, our results for fractal sprays extend to higher dimensions the pointwise tube formula for (1-dimensional) fractal strings obtained earlier by Lapidus and van Frankenhuijsen. Our pointwise tube formulas are expressed as a sum of the residues of the "tubular zeta function" of the fractal spray in $\mathbb{R}^d$. This sum ranges over the complex dimensions of the spray, that is, over the poles of the geometric zeta function of the underlying fractal string and the integers $0,1,...,d$. The resulting "fractal tube formulas" are applied to the important special case of self-similar tilings, but are also illustrated in other geometrically natural situations. Our tube formulas may also be seen as fractal analogues of the classical Steiner formula.

==> residues-of-gzT.tex <==
%%!TEX root = pointwise.tex

\section{TO BE REMOVED}%Residues of the tubular zeta functions \gzT and \gzG}
\label{Xsec:residues-of-gzT}

The following result is an immediate consequence of \cite[Thm.~3.6]{FGCD}, which provides the structure of the complex dimensions of self-similar fractal strings (even for the case when \abscissa may be larger than 1).


\begin{defn}\label{Xdef:Minkowski-measurable}
  Let \abscissa denote the unique real solution of \eqref{eqn:Moran}, often called the \emph{similarity dimension} of $\attr$.
  %\footnote{Since the definition of a self-similar tiling requires $\simtset$ to satisfy the open set condition, \abscissa coincides with the Minkowski and Hausdorff dimension of $F$.} 
  %
  We define a self-similar tiling \tiling to be \emph{Minkowski measurable} iff
  \linenopax
    \begin{align}
      \label{Xdef:Mink meas}
      0 < \lim_{\ge \to 0^+} V(\tiling,\ge) \ge^{-(d-\abscissa)} < \iy,
    \end{align}
    i.e., if the limit in \eqref{Xdef:Mink meas} exists \emph{and} takes a value in $(0,\iy)$.
\end{defn}

Much of the information in Remark~\ref{rem:Minkowski-warmup} is needed in the proof (or the statement) of the results concerning Minkowski measurability in this subsection.




\subsection{Minkowski measurability of self-similar tilings}
\label{Xsec:Minkowski-measurability}

In this subsection, we apply our pointwise tube formula \eqref{eqn:pointwise-tube-formula}, along with earlier results and techniques from \cite[\S3 and \S8.4]{FGCD} (see especially Thm.~3.6, Thm.~3.25 and Thm.~5.1), in order to deduce several results concerning the Minkowski measurability (or lack thereof) of self-similar tilings.

We first need to provide definitions of Minkowski measurability and content of self-similar tilings, as some terminology is slightly nonstandard. (This minor deviation is justified by the resulting convenience in the sequel.)

\begin{defn}[Minkowski content and dimension]
  \label{Xdef:Minkowski-content-and-dimension}
  Let \tiling be a self-similar tiling. 
  The \emph{(inner) Minkowski dimension} of \tiling is the real number $\abscissa_\tiling \geq 0$ given by
  \linenopax
  \begin{align}\label{Xeqn:Minkowski-dimension}
    \abscissa_\tiling 
    %:=& \inf\{\ga \geq 0 \suth \Mink_\ga(\tiling) = 0\} \notag \\
    :=& \inf\{\ga \geq 0 \suth V(\tiling,\ge) = O(\ge^{d-\ga}), \text{ as } \ge \to 0^+\}.
  \end{align}
  Then the \emph{upper Minkowski content} and the \emph{lower Minkowski content} of \tiling are given by
  \linenopax
  \begin{align}
    \Minku(\tiling)
    &:= \limsup_{\ge \to 0^+} V(\tiling,\ge) \ge^{-(d-\abscissa_\tiling)}
      \text{, and }\label{Xeqn:upper-Minkowski-content} \\
%  \end{align}
%  is
%  \linenopax
%  \begin{align}
\label{Xeqn:lower-Minkowski-content}
    \Minkl(\tiling)
    &:= \liminf_{\ge \to 0^+} V(\tiling,\ge) \ge^{-(d-\abscissa_\tiling)},
  \end{align}
  respectively. Clearly, one has 
  %\linenopax
  %\begin{align}\label{Xeqn:lower<=upper-content}
  $  0 \leq \Minkl(\tiling) \leq \Minku(\tiling) \leq \iy.$
  %\end{align}
  When this takes the form
  \linenopax
  \begin{align}\label{Xeqn:lower=upper-content}
    0 < \Minkl(\tiling) = \Minku(\tiling) < \iy,
  \end{align}
  we say that \tiling is \emph{Minkowski measurable}, and that \tiling has \emph{Minkowski content} $\Mink(\tiling) := \Minkl(\tiling) = \Minku(\tiling)$. 
  More precisely, if the limit 
  \linenopax
  \begin{align}\label{Xeqn:Minkowski-content}
    \Mink_\ga(\tiling) 
    := \lim_{\ge \to 0^+} \ge^{-(d-\ga)} V(\tiling, \ge)
  \end{align}
  exists and takes a value in $[0,\iy)$, then one says that the \emph{\ga-dimensional Minkowski content} of \tiling exists. In this case, $\abscissa_\tiling 
  = \inf\{\ga \geq 0 \suth \Mink_\ga(\tiling) = 0\}$. %, then $\Mink_\ga(\tiling)$ is called. 
  In general, discussion of $\Mink(\tiling)$ or $\Mink_\ga(\tiling)$ tacitly implies that the corresponding limit %\eqref{Xeqn:Minkowski-content} 
  exists.
  %
  %
  %If $0 < \Mink_\ga(\tiling) < \iy$ for some $\ga \geq 0$, then we must have $\ga = \abscissa_\tiling$ and then \tiling is said to be \emph{Minkowski measurable}. 
  %
\end{defn}

The next definition is adapted from \cite[Def.~8.29]{FGCD} and will be useful in the case of lattice self-similar tilings.

\begin{defn}[Average Minkowski content]
  \label{Xdef:Average-Minkowski-content}
  Let \tiling be a self-similar tiling, and fix $\ga \geq 0$. If the limit
  \linenopax
  \begin{align}\label{Xeqn:alpha-average-Minkowski-content}
    \Minka_\ga (\tiling)
    := \lim_{T \to \iy} \frac1{\log T} \int_{1/T}^1 \ge^{-(d-\ga)} V(\tiling,\ge) \frac{d\ge}{\ge}
  \end{align}
  exists and takes a value in $[0,\iy)$, then $\Minka_\ga (\tiling)$ is called the \emph{\ga-dimensional average Minkowski content} of \tiling and is said to exist.
  %
  Furthermore, if 
  \linenopax
  \begin{align}\label{Xeqn:average-Minkowski-content}
    0 < \Minka_\ga(\tiling) < \iy
  \end{align}
  for $\ga = \abscissa_\tiling$, then $\Minka = \Minka_\ga(\tiling)$ is called the \emph{average Minkowski content} of \tiling.
\end{defn}

\begin{remark}\label{Xrem:Minkowski-for-sets}
  Definitions~\ref{Xdef:Minkowski-content-and-dimension} and \ref{Xdef:Average-Minkowski-content} have an obvious counterpart for any bounded set $A \ci \bRd$, and in particular, for the generator \gen of \tiling and the associated self-similar set \attr. For example, in the sequel, $\abscissa_\gen$ and $\Mink(\gen)$, denote respectively the Minkowski dimension and the Minkowski content of \gen, etc. 
\end{remark}

\begin{remark}\label{Xrem:D_T-is-not-D}
  We caution the reader that we do not always have $\abscissa_\tiling = \abscissa$, where $\abscissa=\abscissa_\sL$ is given by \eqref{eqn:D-dimensions}; see Theorem~\ref{Xthm:self-similar-tilings-of-maximal-dimension}. In Theorem~\ref{Xthm:characterization-of-Minkowski-measurability}, we give conditions under which this equality does hold.
\end{remark}

%We are now ready to discuss the Minkowski measurability of self-similar tilings.

In the remainder of this section, \tiling is assumed to be a self-similar tiling with a single generator \gen for which a Steiner-like representation has been specified (as in \eqref{eqn:def-prelim-Steiner-like-formula}) and which is scaled by the self-similar string \sL.

Theorem~\ref{Xthm:characterization-of-Minkowski-measurability} is a special case of a more general and complicated theorem, but it is sufficiently simple and appealing that we wish to single it out.%
  %
  \footnote{It may also seem familiar to someone acquainted with the theory of self-similar strings, as developed in \cite[Chap.~2--3]{FGCD}.}
  %
In order to simplify its statement, we introduce the following hypothesis.

\begin{defn}\label{Xdef:HD}
  The Steiner-like representation of \gen satisfies condition \ref{Xeqn:H_D} if $\crv_d(\gen) = 0$ and $d-1 < \abscissa < d$ with
  \linenopax
  \begin{align}
    \label{Xeqn:H_D} \tag*{$\mathbf{H_D}$}
    M_\abscissa(\gen) > 0 \q\text{and}\q |f_d(\gen,\ge)| \leq C \ge^{\gt_d},
    \text{ for } 0 < \ge \leq \genir,
    %\crv_d(\gen,\ge) = O(\ge^{\gt_d}), \text{ as } \ge \to 0^+,
    %\qq \text{ and } \qq M_\abscissa(\gen) > 0,
  \end{align}
  for some constants $C>0$ and $\gt_d$ with $0 < \gt_d < d-\abscissa$ and 
  \linenopax
  \begin{align}\label{Xeqn:M_D(G)}
    M_\abscissa(\gen) = \sum_{k=0}^{d-1} \frac{\genir^{\abscissa-k}}{\abscissa-k} (d-k) \crv_k(\gen). 
  \end{align}
\end{defn}
  Since $f_d(\ge) := \crv_d(\gen,\ge) - \crv_d(\gen)$, the 
  upper bound on $|f_d(\ge)|$ assumed in \ref{Xeqn:H_D} implies a similar one for $|\crv_k(\gen,\ge)|$.
  %decay condition on $\crv_d(\gen,\ge)$ assumed in \ref{Xeqn:H_D} is equivalent to assuming that $f_d(\ge) = O(\ge^{\gt_d})$, as $\ge \to 0^+$. 
  Note that by \eqref{eqn:def-prelim-Steiner-like-formula}, we must always have $\lim_{\ge \to 0^+} \crv_d(\gen,\ge) = \lim_{\ge \to 0^+} V(\gen,\ge) = 0$. 
  %Consequently, this assumption on the decay of $\crv_d(\gen,\ge)$ is rather mild. In fact, we have $\crv_d(\gen,\mydot) \equiv 0$ in every known example.
  The latter limit, however, is clearly implied by the second requirement in $\mathbf{H_D}$, %(that is, \ref{Xeqn:H_k} for $k=d$) 
  but is not equivalent to it.

In Theorem~\ref{Xthm:characterization-of-Minkowski-measurability}, the terms ``lattice'' and ``nonlattice'' are used as in Proposition~\ref{thm:lattice-nonlattice-dichotomy}.

\begin{theorem}[Characterization of Minkowski measurability for self-similar tilings]
  \label{Xthm:characterization-of-Minkowski-measurability}
  Let \tiling be a self-similar tiling satisfying hypopthesis \ref{Xeqn:H_D}. Then \tiling has Minkowski dimension $\abscissa_\tiling = \abscissa$. Moreover, \tiling is Minkowski measurable if and only if it is nonlattice. More precisely, there is a dichotomy.  
  \hfill \\
  \hstr[3] \emph{Lattice case}. If \tiling is lattice, then it is not Minkowski measurable, but % because it has geometric oscillations of order $\abscissa = \abscissa_\tiling$ in its geometry. 
  \linenopax
  \begin{align}\label{Xeqn:lower<upper-lattice-content}
    0 < \Minkl(\tiling) < \Minku(\tiling) < \iy.
  \end{align}
  However, its average Minkowski content $\Minka(\tiling)$ exists, is positive, and is given by the right-hand side of \eqref{Xeqn:nonlattice-Mink-residue}.
  \hfill \\
  \hstr[3] \emph{Nonlattice case}. If \tiling is nonlattice, then it is Minkowski measurable with Minkowski content satisfying $0 < \Mink_\abscissa(\tiling) < \iy$ and given by 
  \linenopax
  \begin{align}\label{Xeqn:nonlattice-Mink-residue}
    \Mink_\abscissa(\tiling) = \res[\abscissa]{\gzL(s)} \frac{M_\abscissa(\gen)}{d-\abscissa},
  \end{align}
  where $M_\abscissa(\gen)$ is as in \eqref{Xeqn:M_D(G)} and $\res[\abscissa]{\gzL(s)}$ is as in \eqref{eqn:nonlattice-residues}. 
\end{theorem}

\begin{remark}\label{Xrem:proofs-of-Minko-theorems}
  %As was mentioned earlier, 
  Theorem~\ref{Xthm:characterization-of-Minkowski-measurability} (and Theorem~\ref{Xthm:self-similar-tilings-of-maximal-dimension}) follows from a more general theorem which distinguishes all possible cases, each of which is proved in much the same manner (once certain residues have been computed). For this reason, we give only the proof of Theorem~\ref{Xthm:characterization-of-Minkowski-measurability}, as this covers the most interesting situation.%
  %\footnote{In the case of Theorem~\ref{Xthm:self-similar-tilings-of-maximal-dimension}, the main difference is that the integer dimensions $d$ (which is not in $\sD_\tiling$) contributes a nonzero constant terms to the tube formula, equal to $\crv_d(\gen) \gzL(d) = \res{\gzT(\ge,s)} + \gl_d(\gen) \gzL(d)$.} 
  This proof relies heavily on the error term \eqref{eqn:pointwise-error} of the pointwise formula \eqref{eqn:pointwise-tube-formula} applied to the self-similar tiling \tiling, and also uses results about generalized self-similar strings appearing in \cite[Thm.~3.6, Thm.~3.25, Thm.~5.17 and \S8.4]{FGCD}. In order not to interrupt the flow of the paper, the proof of Theorem~\ref{Xthm:characterization-of-Minkowski-measurability} (and Corollary~\ref{Xthm:Minkowski-measurable-for-attractor}, below) is postponed until the end of this section. 
\end{remark}

%Theorem~\ref{Xthm:self-similar-tilings-of-maximal-dimension} is also a special case of a more general theorem. 

\begin{theorem}[Self-similar tilings of maximal dimension]
  \label{Xthm:self-similar-tilings-of-maximal-dimension}
  Assume that \tiling is a self-similar tiling such that $\crv_d(\gen) \neq 0$,%
  %
  \footnote{In other words, we assume $\crv_d(\gen) > 0$. The fact that we must always have $\crv_d(\gen) \geq 0$ is a consequence of the existence of $\Mink_d(\gen)$ in \eqref{Xeqn:Minkowski-content}. 
  %
  } 
  and there exist constants $C>0$ and $0 < \gt_d < d-D$ for which 
  $|\crv_d(\gen,\ge) - \crv_d(\gen)| \leq C \ge^{\gt_d}$ for $0 < \ge \leq \genir$.
  %$\crv_d(\gen,\ge) = \crv_d(\gen) + O(\ge^{\gt_d})$, as $\ge \to 0^+$. 
  Then \tiling and \gen have Minkowski dimension $D_\tiling = D_\gen = d$. 
  Furthermore, \gen is Minkowski measurable with Minkowski content in $(0,\iy)$ given by
  \linenopax
  \begin{align}\label{Xeqn:generator-Mink-content}
    \Mink(\gen) = \Mink_d(\gen) = \crv_d(\gen).
  \end{align}
  Moreover, if \tiling is nonlattice, then \tiling is Minkowski measurable with Minkowski content in $(0,\iy)$ given by
  \linenopax
  \begin{align}\label{Xeqn:Mink(tiling)-factors}
    \Mink(\tiling) = \Mink_d(\tiling) = \gzL(d) \crv_d(\gen).
  \end{align}
  However, if \tiling is lattice, then \tiling is \emph{not} Minkowski measurable but its average Minkowski content $\Minka(\tiling) = \Minka_d(\tiling)$ exists and satisfies \eqref{Xeqn:alpha-average-Minkowski-content} and \eqref{Xeqn:average-Minkowski-content} and, just as in \eqref{Xeqn:Mink(tiling)-factors}, one also has $\Minka(\tiling) = \gzL(d) \crv_d(\gen)$.
\end{theorem}

Recall that for a nontrivial self-similar tiling, we have $D = D_\sL < d$. Hence, $D < D_\tiling$ in Theorem~\ref{Xthm:self-similar-tilings-of-maximal-dimension}.
%  \begin{proof}[Proof of Theorem~\ref{Xthm:self-similar-tilings-of-maximal-dimension}]
%  \end{proof}

\begin{remark}\label{Xrem:proof-of-maxl-dimn-theorem}
  %As was mentioned earlier, Theorem~\ref{Xthm:characterization-of-Minkowski-measurability} and Theorem~\ref{Xthm:self-similar-tilings-of-maximal-dimension} follow from a more general theorem which distinguishes all possible cases, each of which is proved in much the same manner (once certain residues have been computed). For this reason, we give only the proof of Theorem~\ref{Xthm:characterization-of-Minkowski-measurability}, as this covers the most interesting situation.%
  As mentioned in Remark~\ref{Xrem:proofs-of-Minko-theorems}, the proof of Theorem~\ref{Xthm:self-similar-tilings-of-maximal-dimension} is sufficiently similar to the proof of Theorem~\ref{Xthm:characterization-of-Minkowski-measurability} that we omit it. However, in contrast to Theorem~\ref{Xthm:characterization-of-Minkowski-measurability}, where $D_\tiling = D_\sL \neq D_\gen$, Theorem~\ref{Xthm:self-similar-tilings-of-maximal-dimension} discusses the case when $D_\tiling = D_\gen = d > D_\sL$ instead. Indeed, it can be easily verified that in Theorem~\ref{Xthm:self-similar-tilings-of-maximal-dimension}, $D_\gen$ (the Minkowski dimension of \gen) is equal to the largest integer $k \in \{0,1,\dots,d-1\}$ such that $\crv_k(\gen) > 0$, and \gen is Minkowski measurable with Minkowski content $\Mink_k(\gen) = \crv_k(\gen)$.
  %For the reader who wishes to pursue this, let us note that 
  In the proof of Theorem~\ref{Xthm:self-similar-tilings-of-maximal-dimension}, the main difference is that the integer dimension $d$ (which is not in $\sD_\sL$) contributes a nonzero constant terms to the tube formula, equal to $\crv_d(\gen) \gzL(d) = \res[s=d]{\gzT(\ge,s)} + \gl_d(\gen) \gzL(d)$. 
  %This proof relies heavily on the error term \eqref{Xeqn:pointwise-error} of the pointwise formula \eqref{Xeqn:pointwise-tube-formula} applied to the self-similar tiling \tiling, and also uses results about generalized self-similar strings appearing in \cite[Thm.~3.6, Thm.~3.25 and \S8.4]{FGCD}. In order not to interrupt the flow of the paper, the proof of Theorem~\ref{Xthm:characterization-of-Minkowski-measurability} (and Corollary~\ref, below) is postponed until the end of this section. 
\end{remark}

We close the discussion of the main results of \S\ref{Xsec:Minkowski-measurability} with a simple corollary of Theorem~\ref{Xthm:characterization-of-Minkowski-measurability} and the results of \cite{GeometryOfSST} recalled in Remark~\ref{rem:compatibility-theorem}.

\begin{cor}[Minkowski measurability of self-similar sets]
  \label{Xthm:Minkowski-measurable-for-attractor}
  Suppose the tiling \tiling satisfies the hypothesis \ref{Xeqn:H_D}%
  \footnote{Note that by \ref{Xeqn:H_D}, it follows from Theorem~\ref{Xthm:characterization-of-Minkowski-measurability} and Remark~\ref{rem:incarnations-of-D} that $D_\tiling = D_F = D$.}
  and that its self-similar set \attr satisfies the condition \eqref{eqn:compatibility-condition} of the compatibility theorem (\cite[Thm.~6.2]{GeometryOfSST}; see Remark~\ref{rem:compatibility-theorem}) for some feasible open set $O$ with closure $K = \bar{O}$ such that $\Mink_\abscissa(K)$ exists. (It may be $0$, but it must be finite.) 
  Then \attr is Minkowski measurable if and only if \tiling (or equivalently \sL) is nonlattice. In the lattice case, we have
  $0 < \Minkl(\attr) < \Minku(\attr) < \iy$, and similarly for \tiling in place of \attr.
\end{cor}
\begin{proof}
  As above, denote the closure of a feasible open set $O$ by $K = \bar O$ and let $T = \bigcup \simt_w(\gen)$ be the union of the tiles in the self-similar tiling $\tiling(O)$. Consider the (outer) $\ge$-parallel set $\attr_\ge$ of the attractor $\attr$, as defined in \eqref{eqn:ext-nbd-of-A}. From \cite[Thm.~6.2]{GeometryOfSST}, we have the disjoint union $\attr_\ge = T_{-\ge} \cup K_\ge$ whenever $\bd K\ci F$.
  
  We need to say something about the upper \abscissa-dimensional Minkowski content:  
  \linenopax
  \begin{align}\label{Xeqn:Minkowski-content}
    \Minku_\abscissa(K) 
    = \limsup_{\ge \to 0^+} \ge^{D-d} V(K_\ge).  
  \end{align}
  If this is zero, everything is fine, i.e. the \abscissa-dimensional Minkowski content of \attr (in the usual sense) and of the tiling \sT (in the sense of Definition~\ref{Xdef:Minkowski-content-and-dimension}) coincide and Corollary~\ref{Xthm:Minkowski-measurable-for-attractor} holds.  
  If not, then one has to use the fact that, by hypothesis, $\Mink_\abscissa(K)$ exists in $[0,\iy)$:
  %prove the limit in \eqref{Xeqn:Minkowski-content}; to this end, let  
  \linenopax
  \begin{align*}%\label{Xeqn:}
    \Mink_\abscissa(K) = \lim_{\ge \to 0^+} \ge^{D-d} V(K_\ge).  
  \end{align*}
  Suppose \attr is non-lattice. Then $\Mink_\abscissa(T)$ (the Minkowski content of the tiling) and $\Mink_\abscissa(\attr)$ (the Minkowski content of \attr) do exist (by the first sentence of Corollary~\ref{Xthm:Minkowski-measurable-for-attractor} and Gatzouras' result, respectively). Hence, $\Mink_\abscissa(K)$ exists (it may be zero) and  
  \linenopax
  \begin{align}\label{Xeqn:Minkowski-content-decomp}
    \Mink_\abscissa(\attr) = \Mink_\abscissa(T) + \Mink_\abscissa(K).     
  \end{align}
  Suppose \attr is lattice. Then $\Mink_\abscissa(T)$ does not exist (by Corollary~\ref{thm:ptwise-result-self-similar-case-simplified}, first sentence), but for $\Mink_\abscissa(F)$ we do not know.
  
  If $\Mink_\abscissa(K)$ can be shown to exist, then \eqref{Xeqn:Minkowski-content-decomp} implies that $\Mink_\abscissa(F)$ does not exist, as desired.  But what if $\Mink_\abscissa(K)$ does not exist? Maybe we can find some more refined argument in this case. But it is certainly not true in general that the sum of two divergent sequences is divergent as well.  
  
  In conclusion: up to now, the second assertion in Corollary~\ref{Xthm:Minkowski-measurable-for-attractor} is true only with the additional hypothesis that $\Mink_\abscissa(K)$ exists (including the case that $\Mink_\abscissa(K)=0$).
  %
  %Now Proposition~\ref{Xthm:lattice-nonlattice-dichotomy} follows from Theorem~\ref{thm:pointwise-tube-formula} applied to a suitable window, much as in \cite[\S8.4]{FGCD}.
\end{proof}


\subsection{The proof of Theorem~\ref{Xthm:characterization-of-Minkowski-measurability}} \hfill \\
\marginpar{$\leftarrow$ Note for ourselves}
{[[\textsf{The following proof assumes that we have proven the tube formula with a good error term, and a good estimate for the residues of $\gzT[\head]$ at the visible integer dimensions, without the restriction $S(0) < 0$. More specifically, we need to find conditions on the coefficients functions $\crv_k(\gen,\cdot)$ such that for $k=0,1,\dots,d$, each residue satisfies the estimate
\linenopax
\begin{align*}%\label{eqn:}
  \res[s=k]{\gzT[\head](\ge,s)} 
  = O\left(\ge^{d - \sup S}\right),
  \qq \text{ as } \ge \to 0^+.
\end{align*}
This is necessary for a screen $S$ which lies arbitrarily close to the line $\Re s = \abscissa$.}]]}

\begin{proof}[Proof of Theorem~\ref{Xthm:characterization-of-Minkowski-measurability}]
In light of the first part of Proposition~\ref{thm:lattice-nonlattice-dichotomy}, the lattice case is relatively easy, and can be handled exactly like \cite[Thm.~8.23]{FGCD} and \cite[Thm.~8.29]{FGCD}. The remainder of this proof is concerned with the nonlattice case.

According to \cite[Thm.~3.25]{FGCD} (which applies to generalized self-similar strings and which holds even for $\abscissa > 1$), there exists a screen $S$ which lies to the left of the line $\Re s = \abscissa$ such that \gzL is bounded on $S$, and all the visible scaling complex dimensions are simple and have uniformly bounded residues, in the sense that there is a $C>0$ for which
\linenopax
\begin{align}\label{eqn:residue-bound}
  \left|\res{\gzL(s)}\right| \leq C, 
  \qq \text{for all } \pole \in \DL(W),
\end{align}
where $W$ is the window corresponding to $S$.
%
In fact, the screen can be taken to be arbitrarily close to (but bounded away from) the line $\Re s = \abscissa$. More precisely, given an arbitrarily small $\gd > 0$ (so that, in particular, $\gd < \abscissa-(d-1)$), we may assume that except for $\pole \in \{\abscissa,d\}$, all the visible complex dimensions \pole of \tiling lie in 
\linenopax
\begin{align}\label{eqn:polestrip}
  \polestrip_\gd := \{s \in \bC \suth \abscissa - \tfrac\gd2 < \Re s < \abscissa - \tfrac\gd4\}.
\end{align}
Note that this implies that $\sup S \leq \abscissa - \frac\gd4$ and 
\linenopax
\begin{align}\label{eqn:polestrip-cont}
  \polestrip_\gd \ci \{s \in \bC \suth d-1 < \Re s < d\}.
\end{align}

\marginpar{The version we need $\to$}
Recall that the fractal tube formula with error term gives
\linenopax
\begin{align}\label{eqn:Minkowski-characterization-deriv-1}
  V(\tiling,\ge)
  &= \sum_{\pole \in \DL(W)} c_\pole \ge^{d-\pole} 
   + \sum_{k \in \{0,1,\dots,d\} \cap W} (c_k + e_k(\ge)) \ge^{d-k} 
   + \R(\ge),
\end{align}
where $\R(\ge) = O(\ge^{d-\sup S})$ as $\ge \to 0^+$, and with $c_\pole$, $c_k$, and $e_k(\ge)$ as in \eqref{eqn:self-similar-pointwise-tube-formula-coefficients-cw}--\eqref{eqn:self-similar-pointwise-tube-formula-coefficients-ek}. Note that for the latter, \eqref{eqn:self-similar-pointwise-tube-formula-coefficients-ek}, \eqref{eqn:def:f_k}, and \eqref{eqn:residues-of-gzT(ii)} imply that for $k \in \{0,1,\dots,d\}$,
\linenopax
\begin{align}
  \ge^{d-k}e_k(\ge) 
  %&= \sum_{j=1}^{J(\ge)} \scale_j^k \left(\crv_k(\gen, \scale_j^{-1}\ge) - \crv_k(\gen)\right)
  = \res[s=k]{\gzT[\head](\ge,s)}
  = O(\ge^{d-\sup S}),
  \q\text{as } \ge \to 0^+,
  \label{eqn:self-similar-pointwise-tube-formula-coefficients-ek-redux}
\end{align}
where $J(\ge) := \max\{j \geq 1 \suth \scale_j^{-1} \ge < \genir\} \vee 0$ as in \eqref{eqn:J(eps)}.
%
Under the assumptions of Theorem~\ref{Xthm:characterization-of-Minkowski-measurability} (see especially hypothesis \ref{Xeqn:H_D}), we have $d-1 < \abscissa < d$, $\crv_d(\gen) = 0$, and $M_\abscissa(\gen) > 0$. 
%, which implies that $\crv_d(\gen) = 0$. 
Hence, $c_d = \crv_d(\gen) \gzL(d) = 0$. 

%Assume a good estimate for something $\ge^{d-d}e(\ge) = O(\ge^{d-\sup S})$ as $\ge \to 0^+$. 
Also, since each $\pole \in \DL(W)$ is simple and lies in $P_\gd$ (see \eqref{eqn:polestrip}), we have that $\DL(W) \cap \{0,1,\dots,d\} = \es$.
Therefore, there are \emph{no} visible integer dimensions that are poles of \gzT[\head] in this case. %: $\{0,1,\dots,d\} \cap W = \es$. 
Hence, \eqref{eqn:Minkowski-characterization-deriv-1} becomes
\linenopax
\begin{align}\label{eqn:Minkowski-characterization-deriv-2}
  V(\tiling,\ge)
  &= c_\abscissa \ge^{d-\abscissa} + \sum_{\pole \in \DL(W) \cap \polestrip_\gd} c_\pole \ge^{d-\pole} +\R(\ge),
\end{align}
where, in light of \eqref{eqn:gzG[tail]} and \eqref{eqn:residues-of-gzT(i)}, and since $\DL(W)$ and $\{0,1,\dots,d\}$ are disjoint,
\linenopax
\begin{align} 
  c_\pole 
  &= \res{\gzL(s)} \frac{M_\pole(\gen)}{d-\pole},
  \qq \text{for } \pole \in \DL(W),
    \label{eqn:nonlattice-Minkowski-content-gen}
\end{align}
with
\linenopax
\begin{align} 
  M_\pole(\gen) 
  &= \sum_{k=0}^{d-1} \frac{\genir^{\pole-k}}{\pole-k}(d-k) \crv_k(\gen).
    \label{eqn:nonlattice-Minkowski-content-gen-sum}
\end{align}
In particular, 
\linenopax
\begin{align} 
  c_\abscissa 
  &= \res[s=\abscissa]{\gzL(s)} \frac{M_\abscissa(\gen)}{d-\abscissa}
    \label{eqn:nonlattice-Minkowski-content}
\end{align}
upon combining \eqref{Xeqn:M_D(G)} with \eqref{eqn:self-similar-pointwise-tube-formula-coefficients-cw} in the case $\pole=\abscissa$.
%
Note that $c_\abscissa > 0$ since \abscissa is a pole of \gzL, and $M_\abscissa(\gen) > 0$, and that \eqref{eqn:Minkowski-characterization-deriv-2}, in combination with the error estimate $\R(\ge) = O(\ge^{d - \sup S})$, implies that 
\linenopax
\begin{align}\label{eqn:Minkowski-measurability-claim}
  \ge^{-(d-\abscissa)} V(\tiling,\ge)
  &= c_\abscissa + \sum_{\pole \in \DL(W) \cap \polestrip_\gd} c_\pole \ge^{\abscissa-\pole} + O(\ge^{\abscissa-\sup S}),
  \qq \text{as } \ge \to 0^+.
\end{align}
%
Note that since $\sup S \leq \abscissa - \frac\gd4$, we have that $\abscissa - \sup S \geq \frac\gd4$, and hence that
\linenopax
\begin{align}\label{eqn:order-est}
  O\left(\ge^{\abscissa-\sup S}\right) = O(\ge^{\gd/4}) = o(1), 
  \qq\text{as } \ge \to 0^+.   
\end{align}


To see that \tiling is Minkowski measurable, we show that the sum in \eqref{eqn:Minkowski-measurability-claim} is absolutely convergent and tends to $0$ as $\ge \to 0^+$; see Definition~\ref{Xdef:Minkowski-content-and-dimension}. However, \eqref{eqn:nonlattice-Minkowski-content-gen} implies
\linenopax
\begin{align*}%\label{eqn:}
  |c_\pole| \leq C \frac{|M_\pole(\gen)|}{|d-\pole|},
  \qq \text{for } \pole \in \DL(W),
\end{align*}
where the positive constant $C$ is as in \eqref{eqn:residue-bound}.
%
Therefore, for a fixed $\ge > 0$, the sum in \eqref{eqn:Minkowski-measurability-claim} can be compared to 
\linenopax
\begin{align}\label{eqn:polestrip-sum}
  \sum_{\pole \in \polestrip_\gd} \frac1{|\pole|^{d+1}},
\end{align}
which converges by the density estimate \cite[(3.10)]{FGCD}, according to which the poles of \gzL have a \emph{linear} density. In other words, \eqref{eqn:polestrip-sum} converges because $\sum_{n=1}^\iy \frac1{n^{d+1}} < \iy$ for any $d \geq 1$.

This argument enables us to apply the method of proof from \cite[Thm.~5.17]{FGCD} to deduce that
\linenopax
\begin{align*}%\label{eqn:}
  \sum_{\pole \in \DL(W) \cap \polestrip_\gd} c_\pole \ge^{\abscissa - \pole} = o(1),
  \qq\text{as } \ge \to 0^+,
\end{align*}
in addition to the fact that this sum converges for each fixed $\ge > 0$. Consequently, \eqref{eqn:Minkowski-measurability-claim} and \eqref{eqn:order-est} imply that
\linenopax
\begin{align}\label{eqn:Minkowski-measurability-nonlattice-satisfied}
  \ge^{-(d-\abscissa)} V(\tiling,\ge)
  = c_\abscissa + o(1),
  \qq \text{as } \ge \to 0^+,
\end{align}
and since $0 < c_\abscissa < \iy$, we conclude that \tiling is Minkowski measurable with Minkowski content equal to $c_\abscissa$. 
\end{proof}



\subsection{Residues of \gzT and \gzG}
  
In this appendix, we introduce \gzG, the tubular zeta function of the generator, and compute the residues of its head and tail decomposition. In \S\ref{Xsec:The-tubular-zeta-function-of-the-generator}, we verify directly that $V(\gen,\ge)$ is given by an exact tube formula and use some of these results in \S\ref{Xsec:residues-of-gzT} to calculate and study the residues of the tubular zeta function \gzT of a self-similar tiling \tiling with generator \gen. Apart from the fact that a self-similar tiling satisfies $\abscissa = \abscissa_\sL < d$ and the only real pole of \gzL is \abscissa itself, all results of this appendix can be easily adapted to any fractal spray based on \gen.

\subsubsection{The tubular zeta function of the generator}
\label{Xsec:The-tubular-zeta-function-of-the-generator}

In the sequel, we let $\gzG(\ge,s)$ denote the tubular zeta function of the generator \gen, where \gen is assumed to have a Steiner-like representation as in \eqref{eqn:def-prelim-Steiner-like-formula}. 
It is defined exactly as $\gzT(\ge,s)$, except that the associated fractal string is given by $\{L_j\}_{j=1}^\iy$ with $L_1 = 1$ and $L_j = 0$ for all $j \geq 2$. In other words, it is the tubular zeta function of the trivial fractal spray with generator \gen.

Exactly as in \eqref{eqn:volume-zeta-split2}, we write 
  \linenopax
  \begin{align}\label{Xeqn:gzG-decomp}
    \gzG = \gzG[\head] + \gzG[\tail].
  \end{align}
%Note that for 
%  \begin{align}\label{Xeqn:J_G(eps)}
%    J_\gen(\ge) := \max\{j \geq 1 \suth \ge < L_j \genir\},  
%  \end{align}
%  we have $J_G(\ge) = 1$ for $0 < \ge < \genir$ and $J_\gen(\ge) := 0$ for $\ge \geq \genir$, by convention. 
It thus follows from \eqref{eqn:volume-zeta-split2} (applied to the trivial fractal spray on \gen) that for $s \in \bC$,
  \linenopax
  \begin{align}\label{Xeqn:gzG[head]}
    \gzG[\head](\ge,s) = \ge^{d-s} \sum_{k=0}^d \frac{\genir^{s-k}}{s-k} f_k(\ge),
    \qq \text{for }\, 0 < \ge < \genir, 
  \end{align}
  with $f_k(\ge) = \crv_k(\gen,\ge) - \crv_k(\gen)$ defined as in \eqref{eqn:def:f_k} for $k=0,1,\dots,d$, and 
  \linenopax
  \begin{align*}%\label{Xeqn:}
    \gzG[\head](\ge,s) = 0,
    \qq\text{for }\, \ge \geq \genir.
  \end{align*}
  Furthermore, for all $\ge > 0$ and $s \in \bC$, we have
  \linenopax
  \begin{align}\label{Xeqn:gzG[tail]}
    \gzG[\tail](\ge,s) = \frac{\ge^{d-s}}{d-s} M_s(\gen),
  \end{align}
  where
  \linenopax
  \begin{align}\label{Xeqn:M_s(G)}
    M_s(\gen) := \sum_{k=0}^{d-1} \frac{\genir^{s-k}}{s-k} (d-k)\crv_k(\gen).
  \end{align}

In light of \eqref{Xeqn:gzG-decomp}--%, \eqref{Xeqn:gzG[head]}, \eqref{Xeqn:gzG[tail]} and 
\eqref{Xeqn:M_s(G)}, for $0 < \ge < \genir$, each of $\gzG[\head](\ge,\mydot)$, $\gzG[\tail](\ge,\mydot)$ and $\gzG(\ge,\mydot)$ is meromorphic in all of \bC, with poles contained in $\{0,1,\dots,d\}$; hence, the set of ``complex dimensions'' of \gen consists of the integer dimensions $\{0,1,\dots,d\}$. Moreover, all of these poles are simple.

\begin{lemma}\label{Xthm:gzG-residues}
  For $0 < \ge < \genir$,
  \linenopax
  \begin{align}\label{Xeqn:gzG[head]-residue-at-k}
    \res[s=k]{\gzG[\head](\ge,s)} = \ge^{d-k} f_k(\ge),
  \end{align}
  for all $k=0,1,\dots,d$, while for $\ge > 0$, 
  \linenopax
  \begin{align}\label{Xeqn:gzG[tail]-residue-at-k}
    \res[s=k]{\gzG[\tail](\ge,s)} = \ge^{d-k} \crv_k(\gen)
  \end{align}
  for $k=0,1,\dots,d-1$, and
  \linenopax
  \begin{align}\label{Xeqn:gzG[tail]-residue-at-d}
    \res[s=d]{\gzG[\tail]} = \crv_d(\gen) - \gl_d(\gen).
  \end{align}
  \begin{proof}
    In view of \eqref{Xeqn:gzG[head]}--\eqref{Xeqn:M_s(G)}, the proof of \eqref{Xeqn:gzG[head]-residue-at-k} and \eqref{Xeqn:gzG[tail]-residue-at-k} is straightforward. To show \eqref{Xeqn:gzG[tail]-residue-at-d}, simply note that by \eqref{Xeqn:gzG[tail]} and \eqref{Xeqn:M_s(G)} (and since $d$ is a simple pole),
    \linenopax
    \begin{align*}%\label{Xeqn:}
      \res[s=d]{\gzG[\tail](\ge,s)}
      &= \lim_{s \to d} (s-d) \gzG[\tail](\ge,s) \\
      &= - \sum_{k=0}^{d-1} \frac{\genir^{d-k}}{d-k} (d-k) \crv_k(\gen) \\
      &= - \left(\gl_d(\gen) - \crv_d(\gen)\right),
      %&= \crv_d(\gen) - \gl_d(\gen),
    \end{align*}
    where we have used \eqref{eqn:leb-coeff-rel} in the last equality.
  \end{proof}
\end{lemma}



\begin{comment}\label{Xrem:monophase-gzG}
  Note that if \gen is monophase (cf.~Remark~\ref{rem:monophase}), its coefficient functions $\crv_k(\gen,\ge)$ are constant (and equal to $\crv_k(\gen)$). Consequently, the functions $f_k$ in \eqref{eqn:def:f_k} vanish identically, and hence so does $\gzG[\head](\ge,s)$ in \eqref{Xeqn:gzG[head]}. As a result, one has $\gzG = \gzG[\tail]$. This is the case, in particular, when $d = 1$ and \gen is a bounded interval (i.e., in the case of a fractal string).
\end{comment}



\subsubsection{The residues of \gzT}
\label{Xsec:residues-of-gzT}

Let \tiling be a self-similar tiling with a fractal string $\sL = \{\scale_j\}_{j=1}^\iy$ and a single generator \gen for which a Steiner-like representation has been fixed. Let $\gzT = \gzT(\ge,s)$ denote the tubular zeta function of \tiling, and let $\gzT = \gzT[\head] + \gzT[\tail]$ be its head--tail decomposition, as in \S\ref{sec:splitting}. 
%Clearly, for any $\ge > 0$ and $\pole \in \bC$, we have
%  \begin{align}\label{eqn:}
%    \res{\gzT(\ge,s)}
%    = \res{\gzT[\head](\ge,s)} + \res{\gzT[\tail](\ge,s)}
%  \end{align}

In light of \eqref{eqn:volume-zeta-split2}, we deduce from \eqref{Xeqn:gzG[tail]} and \eqref{eqn:M_s(G)} that $\gzT[\tail]$ factors as follows:
  \linenopax
  \begin{align}\label{Xeqn:gzT[tail]-factored}
    \gzT[\tail](\ge,s) = \gzG[\tail](\ge,s) \gzL(s)
  \end{align}
Furthermore, still by \eqref{eqn:volume-zeta-split2}, 
  \linenopax
  \begin{align}\label{Xeqn:gzT[head]-notfactored}
    \gzT[\head](\ge,s)
    = \ge^{d-s} \sum_{k=0}^d \frac{\genir^{s-k}}{s-k} 
      \sum_{j=1}^{J(\ge)} \scale_j^s f_k(\scale_j^{-1} \ge),
  \end{align}
  with $f_k$ as in \eqref{eqn:def:f_k} and $J(\ge)$ as in \eqref{eqn:J(eps)}, as usual. % (not to be confused with $J_\gen(\ge)$ in \eqref{Xeqn:J_G(eps)}).
  %More explicitly, we have $f_k(\ge)$
  Recall that $J(\ge) \to \iy$ monotonically as $\ge \to 0^+$, since $\scale_j$ decreases monotonically to $0$ as $j \to \iy$.
  %
\begin{remark}\label{Xrem:gzT[head]-notfactored}
  Observe that \eqref{Xeqn:gzT[head]-notfactored} is not at all the counterpart of the factorization given in \eqref{Xeqn:gzT[tail]-factored}. Indeed, it clearly does not enable us to write $\gzT[\head]$ as the product of $\gzG[\head]$ and \gzL (which would be false). 
  %This fact is the source of some difficulty that will be clearly dealt with in Lemma~\ref{Xthm:residues-of-gzT} and Lemma~\ref{Xthm:residue-decay-rate}.
  
\end{remark}

\begin{remark}\label{Xrem:monophase-gzG}
  Note that if \gen is monophase (cf.~Remark~\ref{rem:monophase}), its coefficient functions $\crv_k(\gen,\ge)$ are constant (and equal to $\crv_k(\gen)$). Consequently, the functions $f_k$ in \eqref{eqn:def:f_k} vanish identically, and hence so does $\gzG[\head](\ge,s)$ in \eqref{Xeqn:gzG[head]}. As a result, one has $\gzG = \gzG[\tail]$. This is the case, in particular, when $d = 1$ and \gen is a bounded interval (i.e., in the case of a fractal string). 
  As a result, the contributions of the residues of the head tubular zeta functions $\gzT[\head]$ vanish identically and thus do not have to be taken into account. This explains, in particular, why the counterpart of Lemma~\ref{Xthm:residue-decay-rate} did not have to be considered in \cite{TFCD} (or in \cite{FGCD}).  
\end{remark}
  %
  Clearly, \eqref{Xeqn:gzT[tail]-factored} implies that for each fixed $\ge > 0$, $\gzT[\head]$ is a meromorphic function on all of \bC, with simple poles lying in $\{0,1,\dots,d\}$. As was noted earlier, the same is true of $\gzG(\ge,s)$. Hence, for all $\pole \in \bC \less\{0,1,\dots,d\}$, we have 
  \linenopax
  \begin{align}
    \res{\gzT(\ge,s)} &= \res{\gzT[\tail](\ge,s)} 
    \label{Xeqn:res(gzT)=res(gzT[tail])} 
  \end{align}
  and
  \linenopax
  \begin{align}
    \res{\gzG(\ge,s)} &= \res{\gzG[\tail](\ge,s)}. 
    \label{Xeqn:res(gzG)=res(gzG[tail])} 
  \end{align}
Furthermore, in light of \eqref{Xeqn:gzG[tail]}, \eqref{Xeqn:M_s(G)} and \eqref{Xeqn:gzT[tail]-factored}, $\gzT[\tail]$ is meromorphic in all of \bC with poles lying in $\sD_\tiling$.
   
We now exploit the factorization \eqref{Xeqn:gzT[tail]-factored} to give the following key result. Note that in this next lemma, we assume that all the poles of $\gzT(\ge,s)$ are simple. Since we are assuming \tiling is self-similar, this means precisely that all the poles of \gzL are simple and that $\abscissa \notin \{0,1,\dots,d\}$.
%$\sD_\sL$ and $\{0,1,\dots,d\}$ are disjoint, i.e., 
%\footnote{Note that since the only real pole of \gzL is $\abscissa = \abscissa_\sL$, and $\abscissa<d$ (since \tiling is self-similar), the only way that \pole could belong to both $\sD_\sL$ and $\{0,1,\dots,d\}$ would be if $\pole = \abscissa = k$, for some $k \in \{0,1,\dots,d-1\}$.} 

\begin{lemma}[Residues of \gzT]
  \label{Xthm:residues-of-gzT}
  Fix $\ge > 0$ and assume that all the poles of $\gzT(\ge,s)$ are simple. Then
  \begin{enumerate}[(i)]
    \item For $\pole \in \sD_\sL$, the residue $\res{\gzT(\ge,s)}$ is given by
      \linenopax
      \begin{align}\label{Xeqn:residues-of-gzT(i)}
        \gzG[\tail](\ge,\pole) \res{\gzL(s)}
        = \frac{\ge^{d-\pole}}{d-\pole} \res{\gzL(s)} M_\pole(\gen),
      \end{align}
      with 
      \linenopax
      \begin{align}\label{eqn:M_w(G)}
        M_\pole(\gen)
        = \sum_{k=0}^{d-1} \frac{\genir^{\pole-k}}{\pole-k} (d-k) \crv_k(\gen)
      \end{align}
      as in \eqref{Xeqn:M_s(G)}.
    \item For $\pole = k \in \{0,1,\dots,d\}$, the residue $\res[s=k]{\gzT[\tail](\ge,s)}$ is given by 
      \linenopax
      \begin{align}\label{Xeqn:residues-of-gzT(ii)}
        \res[s=k]{\gzT[\tail](\ge,s)} 
        = \begin{cases}
          \ge^{d-k} \crv_k(\gen) \gzL(k), & k \neq d, \\
          \left(\crv_d(\gen) - \gl_d(\gen) \right) \gzL(d), &k=d,
        \end{cases}
      \end{align}
      where $\gzL(k) = \left(1 - \sum_{n=1}^N r_n^k\right)^{-1}$, since \tiling is self-similar.%
      %
      \footnote{Note that $\gzL(k) > 0$ if $k > \abscissa $, whereas $\gzL(k) < 0$ if $k < \abscissa$. Indeed, we have $\gzL(k) = (1-\gf(k))^{-1}$, where $\gf(x) := \sum_{n=1}^N r_n^x$. Furthermore, \gf is strictly decreasing on $(0,\iy)$, and $\gf(D) = 1$ by Remark~\ref{rem:incarnations-of-D}.}
      %
    \item For $\pole = k \in \{0,1,\dots,d\}$, the residue $\res[s=k]{\gzT[\head](\ge,s)}$ is given by
      \linenopax
      \begin{align}\label{Xeqn:residues-of-gzT(iii)}
        \res[s=k]{\gzT[\head](\ge,s)} 
        = \ge^{d-k} \sum_{j=1}^{J(\ge)} \scale_j^k f_k(\scale_j^{-1} \ge)
        = \ge^{d-k} e_k(\ge)
      \end{align}
      with $J(\ge)$ as in \eqref{eqn:J(eps)}, $f_k$ as in \eqref{eqn:def:f_k}, and $e_k(\ge)$ as in \eqref{eqn:self-similar-pointwise-tube-formula-coefficients-ek}.
    \item For $\pole \in \bC \less \{0,1,\dots,d\}$, in particular, for $\pole \in \sD_\sL$, we have
      \linenopax
      \begin{align}\label{Xeqn:residues-of-gzT(iv)}
        \res{\gzT[\head](\ge,s)} = 0.
      \end{align}
      %while for $\pole \in \bC \less \sD_\sL$
  \end{enumerate}
  \begin{proof}
    In light of the factorization formula \eqref{Xeqn:gzT[tail]-factored}, and since each $\pole \in \sD_\tiling$ is (at most) a \emph{simple} pole of $\gzT(\ge,s)$,
    \eqref{Xeqn:residues-of-gzT(i)} follows from \eqref{Xeqn:res(gzT)=res(gzT[tail])} and \eqref{Xeqn:gzG[tail]}--\eqref{Xeqn:M_s(G)}, while \eqref{Xeqn:residues-of-gzT(ii)} follows from \eqref{Xeqn:gzG[tail]-residue-at-k}--\eqref{Xeqn:gzG[tail]-residue-at-d} of Lemma~\ref{Xthm:gzG-residues}. Since $\pole = k \in \{0,1,\dots,d\}$ is a simple pole of $\gzT[\head]$, 
    \linenopax
    \begin{align}\label{Xeqn:res(gzThead(k))}
      \res[s=k]{\gzT[\head](\ge,s)} = \lim_{s \to k} (s-k) \gzT[\head](\ge,s),
    \end{align}
    and hence \eqref{Xeqn:residues-of-gzT(iii)} follows immediately from \eqref{Xeqn:gzT[tail]-factored}. Finally, as was already observed, the poles of $\gzT[\head]$ and $\gzT[\tail]$ belong to $\{0,1,\dots,d\}$ and $\sD_\tiling$, respectively.
  \end{proof}
\end{lemma}

\begin{remark}\label{Xrem:sum-of-the-residues}
   Of course, under the assumptions of Lemma~\ref{Xthm:residues-of-gzT}, it follows that in order to calculate $\res[s=k]{\gzT(\ge,s)}$ when $k \in \{0,1,\dots,d\}$, it suffices to add the right-hand sides of \eqref{Xeqn:residues-of-gzT(ii)} and \eqref{Xeqn:residues-of-gzT(iii)}.
\end{remark}

\begin{remark}\label{Xrem:a-complex-dimension-at-k}
  We leave it to the extremely interested reader to determine the residue of $\gzT[\tail](\ge,s)$ at $s=k \in \sD_\sL \cap \{0,1,\dots,d\}$ (under the assumptions of Lemma~\ref{Xthm:residues-of-gzT}), thereby supplementing part (ii) of Lemma~\ref{Xthm:residues-of-gzT}. Since $k$ would be a double pole of $\gzT[\tail]$ in this case, the expression of the resulting residue would involve $\ge \log \ge$, $\res[s=k]{\gzL(s)}$, $\res[s=k]{\gzG(s)}$ and $\ge \gzL(k)$, where ``$\gzL(k)$'' denotes the constant term in the principal part of the Laurent expansion of $\gzL$ around $s=k$; compare to \cite[(8.20)]{FGCD} and the text following it.
  
  Note that since \tiling is assumed to be a self-similar tiling here, it can only happen that $s=k \in \sD_\sL \cap \{0,1,\dots,d\}$ if $s = \abscissa = k \in \{1,2,\dots,d-1\}$. For a general fractal spray, however, $\sD_\sL \cap \{0,1,\dots,d\}$ may not contain \abscissa or may be reduced to $\{\abscissa\}$.
  
  When $\pole \in \sD_\sL \less \{0,1,\dots,d\}$ is a multiple pole of \gzL, we also leave it as an exercise to determine the common residue at $s=\pole$ (and more generally, the common principal part of the Laurent expansion around $s = \pole$) of $\gzT[\tail](\ge,s)$ and $\gzT(\ge,s)$, for any $0 < \ge < \genir$. In light of the factorization formula \eqref{Xeqn:gzT[tail]-factored}, the reader can use \cite[(6.14)]{FGCD} (and the discussion surrounding it) as a guide.
\end{remark}

The next result (Lemma~\ref{Xthm:residue-decay-rate}) will be key to showing that the contribution of the residues of $\gzT[\head]$ at the visible integral dimensions can be neglected when determining the Minkowski measurability of \tiling or calculating its Minkowski content (or its average Minkowski content); see Appendix~\ref{Xsec:appB}. In order to formulate it, we need to make the following rather natural hypothesis, which is already implicit in Theorems~\ref{Xthm:characterization-of-Minkowski-measurability} and \ref{Xthm:self-similar-tilings-of-maximal-dimension}. 

\begin{defn}\label{def:H_k}
  Given $k \in \{0,1,\dots,d\}$ such that $k > \abscissa$, the Steiner-like representation of \gen satisfies condition \ref{Xeqn:H_k} if there exist constants $C>0$ and $0 < \gt_k < \abscissa-d$ for which
  \linenopax
  \begin{align}
    \label{Xeqn:H_k} \tag*{$\mathbf{H_k}$}
    |f_k(\ge)| \leq C \ge^{\gt_k}),
    \qq\text{ for } 0 < \ge \leq \genir.
  \end{align}
  %That is, $\crv_k(\gen,\ge) = \crv_k(\gen) + O(\ge^{\gt_k})$, as $\ge \to 0^+$.
\end{defn}

\begin{lemma}\label{Xthm:residue-decay-rate}
  Given $k \in \{0,1,\dots,d\}$ such that $k > D$, assume that the generator \gen of \tiling satisfies hypothesis \ref{Xeqn:H_k} with exponent $\gt_k$. Then
  \linenopax
  \begin{align}\label{Xeqn:residue-decay-rate}
    \res[s=k]{\gzT[\head](\ge,s)} = O(\ge^{d-k+\gt_k}) = o(\ge^{d-k}), 
    \qq \text{ as } \ge \to 0^+,
  \end{align}
  so that $|e_k(\ge)| \leq C \ge^{\gt_k}$ for all $0 < \ge \leq \genir$, where
  \linenopax
  \begin{align}\label{Xeqn:residue-decay-dimension}
    e_k(\ge) 
    := \sum_{j=1}^{J(\ge)} \scale_j^k f_k(\scale_j^{-1}\ge) 
    = \ge^{-(d-k)} \res[s=k]{\gzT[\head](\ge,s)}.
  \end{align}
  In particular, $\lim_{\ge \to 0^+} e_k(\ge) = 0$.
  \begin{proof}
    Fix \gq such that $0 < \gq < (k-\abscissa) - \gt_k$. According to \ref{Xeqn:H_k}, there exists a constant $C > 0$ such that for all $j \geq 1$%
    \footnote{Recall that since $\sL = \{\scale_j\}_{j=1}^\iy$ is nonincreasing and $\scale_1=1$, we have $\scale_j \leq 1$ for all $j=1,2,\dots$.}
    \linenopax
    \begin{align}\label{Xeqn:f-scale-estimate}
      \scale_j^k \left| f_k(\scale_j^{-1} \ge) \right|
      &\leq C \scale_j^{k-\gt_k} \ge^{\gt_k}
       \leq C \scale_j^{\abscissa+\gq} \ge^{\gt_k},
    \end{align}
    where the second inequality holds because $\abscissa+\gq < k-\gt_k$. Therefore, in light of formula \eqref{Xeqn:residues-of-gzT(iii)} of Lemma~\ref{Xthm:residues-of-gzT}, we have
    \linenopax
    \begin{align}
      \left| \res[s=k]{\gzT(\ge,s)} \right|
      &= \left|\ge^{d-k} \sum_{j=1}^{J(\ge)} \scale_j^k f_k(\scale_j^{-1} \ge) \right| \notag \\
      &\leq \ge^{d-k} \sum_{j=1}^{\iy} \scale_j^k \left|f_k(\scale_j^{-1} \ge) \right| \notag \\
      &\leq C \ge^{d-k} \left(\sum_{j=1}^{\iy} \scale_j^{\abscissa+\gq} \right)\ge^{\gt_k} \notag \\
      &= C \gzL(\abscissa+\gq) \ge^{d-k+\gt_k},
      \label{Xeqn:residue-estimate-k}
    \end{align}
    where the last inequality comes by \eqref{Xeqn:f-scale-estimate}. %
    %\footnote{}
    Since $\abscissa+\gq > \abscissa$, we have $0 < \gzL(\abscissa+\gq) < \iy$. Hence \eqref{Xeqn:residue-decay-rate} follows from \eqref{Xeqn:residue-estimate-k}, and so also does \eqref{Xeqn:residue-decay-dimension}, by \eqref{eqn:self-similar-pointwise-tube-formula-coefficients-ek} and \eqref{Xeqn:residues-of-gzT(iii)}.
  \end{proof}
\end{lemma}

%\begin{remark}\label{rem:lemma-implies-constant}
%  More specifically, the proof of Lemma~\ref{Xthm:residue-decay-rate} implies that
%\end{remark}


\begin{comment}\label{Xrem:residue-estimate-as-e_k}
  The conclusion \eqref{Xeqn:residue-decay-dimension} is equivalent to $\lim_{\ge \to 0^+} e_k(\ge) = 0$, where $e_k(\ge)$ is as in \eqref{eqn:self-similar-pointwise-tube-formula-coefficients-ek}. More precisely, one could say that $e_k(\ge) = O(\ge^{\gt_k})$, as $\ge \to 0^+$.
Note that this equivalent reformulation of \eqref{Xeqn:residue-decay-rate}--\eqref{Xeqn:residue-decay-dimension} follows from the fact that
  \linenopax
  \begin{align}\label{Xeqn:res(s)-as-e_k}
     \res[s=k]{\gzT(\ge,s)}
     = \ge^{d-k} e_k(\ge).
  \end{align}
\end{comment}

\begin{remark}\label{Xrem:asymptotic-behavior-residues}
  A suitable version of Lemma~\ref{Xthm:residue-decay-rate} can also be used to estimate the asymptotic behavior of the contribution to the tube formulas \eqref{eqn:pointwise-tube-formula}, \eqref{eqn:self-similar-pointwise-tube-formula} and \eqref{eqn:self-similar-pointwise-tube-formula-simplified}, coming from the residues of $\gzT[\head](\ge,s)$ as $\ge \to 0^+$, for each visible integer dimension $k \in \{0,1,\dots,d\}$ for which $k > \abscissa$.
\end{remark}

\subsection{Appendix B: Forthcoming}
\label{Xsec:appB}
\hfill \\
\pgap[0.5cm]


